INTERVENOR: Prompting the Coding Ability of Large Language Models with the Interactive Chain of Repair

This paper introduces INTERVENOR (INTERactiVE chaiN Of Repair), a system designed to emulate the interactive code repair processes observed in humans, encompassing both code diagnosis and code repair. INTERVENOR prompts Large Language Models (LLMs) to play distinct roles during the code repair process, functioning as both a Code Learner and a Code Teacher. Specifically, the Code Learner is tasked with adhering to instructions to generate or repair code, while the Code Teacher is responsible for crafting a Chain-of-Repair (CoR) to serve as guidance for the Code Learner. During generating the CoR, the Code Teacher needs to check the generated codes from Code Learner and reassess how to address code bugs based on error feedback received from compilers. Experimental results demonstrate that INTERVENOR surpasses baseline models, exhibiting improvements of approximately 18% and 4.3% over GPT-3.5 in code generation and code translation tasks, respectively. Our further analyses show that CoR is effective to illuminate the reasons behind bugs and outline solution plans in natural language. With the feedback of code compilers, INTERVENOR can accurately identify syntax errors and assertion errors and provide precise instructions to repair codes. All data and codes are available at https://github.com/NEUIR/INTERVENOR

==> figures/codeerror.tex <==
\begin{figure}[t] \centering
    \includegraphics[width=0.4\textwidth]{figures/image/codeerror.pdf}
    \caption{Different error type proportion.} \label{fig:codeerror}
\end{figure}

==> figures/error_description.tex <==
\begin{figure*}[t] \centering
    \includegraphics[scale=0.60]{figures/image/error_description.pdf}
    \caption{Detailed descriptions of each error type in CodeError. We provide an overview of the causes behind each error.} \label{fig:error_description}
\end{figure*}


==> figures/error_distribution.tex <==
\begin{figure*}[t] \centering
    \includegraphics[scale=0.56]{figures/image/error_distribution.pdf}
    \caption{The distribution of error types in CodeError. CodeError covers a total of 9 code error types.} \label{fig:error_distribution}
\end{figure*}


==> figures/repair_type.tex <==
\begin{figure*}[t] \centering
    \includegraphics[scale=0.56]{figures/image/repair_type.pdf}
    \caption{Code repair performance of different methods on CodeError.} \label{fig:repair_type}
\end{figure*}

==> section/4_benchmark.tex <==
\section{CodeError Benchmark}\label{codeerror}
In this section, we introduce CodeError, a code repair benchmark, which consists of codes and error messages. Table \ref{tab:data_statistics} provides a comprehensive overview of the characteristics of the CodeError benchmark. 
Then, we provide insights into the nature of the errors and their distribution. We conduct a statistical analysis of the error types in the buggy code within CodeError, covering a total of 9 types of code errors (see Appendix \ref{app:error_distribution}). The most common error type in CodeError is AssertionError, accounting for 71\% of all errors. Following that are TypeError and NameError, accounting for 13\% and 7\% of the errors, respectively. For explanations of each error, refer to Appendix \ref{app:error_description}.


CodeError benchmark is constructed based on the data collected during the experiments conducted on HumanEval\cite{chen2021evaluating} and MBPP\cite{austin2021program} for code generation. 

In the code generation experiments, given the functional description, the model attempts to generate code that matches the description. 
However, during the testing process, we find various errors in the generated code, including syntax errors, logical errors, and others. In this paper, we use external tools such as the Python interpreter to test the generated code and collect the test results. The code that does not pass the test is considered as buggy code, accompanied by its error messages and test cases, used to construct CodeError.

%\input{figures/benchmark}
As shown in Figure \ref{fig:benchmark}, each entry in CodeError primarily consists of buggy code, error messages, and corresponding test cases.
\begin{itemize}
    \item \textbf{Buggy code} refers to code containing errors. Each buggy code may contain one or more errors.
    \item \textbf{Error messages} include the type of error and a more specific error description. Error types include, but are not limited to, SyntaxError, TypeError, or other types of errors. The error description indicates the potentially erroneous code and a more specific cause of the error.
    \item \textbf{Test} is used to test the corrected code. In CodeError, we use $Pass@k$ as a metric.
\end{itemize}



In this section, We analyze the data statistics of the CodeError benchmark and provide insights into the nature of the errors and their distribution.

\input{tables/coderror_statistic}



==> tables/ablation_study.tex <==

\begin{table*}[]
\centering
\small
\caption{Ablation studies.}
\label{tab:ablation_study}
\begin{tabular}{l|c|c|ccc}
\hline
\multirow{2}{*}{\textbf{Prompting Technique}} & \textbf{HumanEval} & \textbf{MBPP} & \multicolumn{3}{c}{\textbf{HumanEval-X}}      \\
                                              & Python             & Python        & C++           & Java          & JavaScript    \\ \hline
Zero-Shot                                      & 60.3               & 39.8          & 52.4          & 50.6          & 54.3          \\ \hline
+ Code Repair                                 & 67.1               & 51.8          & 57.3          & 59.8          & 62.8          \\
+ COPE ($Iteration=1$)                                  & 69.5               & 51.0          & 59.8          & 65.2          & 60.4          \\
+ COPE ($Iteration=2$)                                  & 73.2               & 54.4          & 61.6          & 67.1          & 62.2          \\
+ COPE ($Iteration=3$)                                  & 75.6               & 56.6          & 65.2          & 68.3          & 64.0          \\
+ COPE ($Iteration=4$)                                  & 75.6               & 57.0          & 66.5          & 68.3          & 64.6          \\
+ COPE ($Iteration=5$)                                  & \textbf{75.6}      & \textbf{57.6} & \textbf{67.1} & \textbf{68.3} & \textbf{67.1} \\ \hline
\end{tabular}
\end{table*}

==> tables/code_generation.tex <==


\begin{table*}[]
\small
\centering
\caption{Code generation results. All values are $Pass@1$, and we use ChatGPT as the foundation model.}
\label{tab:code_generation}
\begin{tabular}{l|c|c|ccc|c}
\hline
\multirow{2}{*}{\textbf{Prompting Technique}} & \textbf{HumanEval}     & \textbf{MBPP}          & \multicolumn{3}{c|}{\textbf{HumanEval-X}}              & \multirow{2}{*}{\textbf{Average}} \\
                                     & Python        & Python        & C++           & Java          & JavaScript    &                          \\ \hline
Zero-shot prompting                  & 60.3          & 39.8          & 52.4          & 50.6          & 54.3          & 51.8                     \\
Zero-shot CoT prompting              & 51.8          & -             & -             & -             & -             & -                        \\
Few-shot prompting                   & 62.2          & -             & -             & -             & -             & -                        \\
CoT prompting                        & 60.4          & -             & -             & -             & -             & -                        \\ \hline
COPE           & \textbf{75.6} & \textbf{57.6} & \textbf{67.1} & \textbf{68.3} & \textbf{67.1} & \textbf{67.1}            \\ \hline
\end{tabular}
\end{table*}

==> tables/code_repair.tex <==
\begin{table}[]
\centering
\small
\caption{Code repair results on CodeError.}
\label{tab:code_repair}
\begin{tabular}{lc}
\hline
\textbf{Prompting Technique} & \textbf{Pass@1} \\ \hline
Zero-shot prompting          & 4.9             \\
Few-shot prompting           & 9.8             \\
CoT prompting                & 9.8             \\
Code Repair w/ Error Type    & 2.8             \\
Code Repair w/ Error Message & 9.8             \\
Code Repair w/ Self-Refine   & 4.6             \\ \hline
INTERVENOR          & \textbf{14.4}   \\ \hline
\end{tabular}
\end{table}

==> tables/code_translation.tex <==

\begin{table*}[]
\centering
\small
\caption{Code translation results. The Zero-Shot values are $Pass@1$, and the reported COPE values underwent only one round of code repair using Chain of Program Repairing. ChatGPT as the foundation model.}
\label{tab:code_translation}
\begin{tabular}{l|cc|cc|cc|cc}
\hline
\multirow{2}{*}{}   & \multicolumn{2}{c|}{\textbf{Python}} & \multicolumn{2}{c|}{\textbf{C++}} & \multicolumn{2}{c|}{\textbf{Java}} & \multicolumn{2}{c}{\textbf{JavaScript}} \\ \cline{2-9} 
                    & Zero-Shot   & COPE                   & Zero-Shot  & COPE                 & Zero-Shot   & COPE                 & Zero-Shot     & COPE                    \\ \hline
\textbf{Python}     & -           & -                      & 62.8       & \textbf{67.7(↑4.9)}  & 70.7        & \textbf{75.1(↑4.4)}  & 82.3          & \textbf{87.8(↑5.5)}     \\
\textbf{C++}        & 81.1        & \textbf{90.2(↑9.1)}    & -          & -                    & 89.6        & \textbf{92.1(↑2.5)}  & 82.3          & \textbf{86.1(↑3.8)}     \\
\textbf{Java}       & 89.6        & \textbf{92.1(↑2.5)}    & 75.6       & \textbf{79.3(↑3.7)}  & -           & -                    & 89.1          & \textbf{90.9(↑1.8)}     \\
\textbf{JavaScript} & 32.3        & \textbf{87.2(↑54.9)}   & 76.2       & \textbf{79.9(↑3.7)}  & 84.8        & \textbf{89.1(↑4.3)}  & -             & -                       \\ \hline
\end{tabular}
\end{table*}
